Data Visceralization: Enabling Deeper Understanding of Data Using Virtual Reality

A fundamental part of data visualization is transforming data to map abstract information onto visual attributes. While this abstraction is a powerful basis for data visualization, the connection between the representation and the original underlying data (i.e., what the quantities and measurements actually correspond with in reality) can be lost. On the other hand, virtual reality (VR) is being increasingly used to represent real and abstract models as natural experiences to users. In this work, we explore the potential of using VR to help restore the basic understanding of units and measures that are often abstracted away in data visualization in an approach we call data visceralization. By building VR prototypes as design probes, we identify key themes and factors for data visceralization. We do this first through a critical reflection by the authors, then by involving external participants. We find that data visceralization is an engaging way of understanding the qualitative aspects of physical measures and their real-life form, which complements analytical and quantitative understanding commonly gained from data visualization. However, data visceralization is most effective when there is a one-to-one mapping between data and representation, with transformations such as scaling affecting this understanding. We conclude with a discussion of future directions for data visceralization.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/6.discussion-old.tex <==
\section{Discussion } \label{sec:discussion}
In this section we generalize findings from our critical reflection, discuss broader aspects of data visceralization, and specify future research opportunities. 

\subsection{Visceral Experiences are Related but Separate from Emotional Experiences}
Visceral experiences may often evoke emotional reactions, such as fear when appearing to look down from a great height---which is one of the reasons why VR has been used for the treatment of psychological disorders. However, for data visceralization, we refer to visceral experiences primarily in terms of the pre-attentive sensory experiences and not the emotions they may or may not evoke. Likewise, many data stories may evoke strong emotional reactions like sadness or anger (e.g. \cite{Halloran:2016:FallenWW2, Lopez:2019:MassShootings}). By treating this phenomena separately, we are focusing primarily on sensory fidelity and are letting the storytelling context convey any desired emotions. 

\subsection{Perceptual Scaling and Truthfulness}
Since we are closely tied to our perceptual sensing, any scaling of inputs into our senses can result in the original data being perceived inaccurately, potentially resulting in experiences that are misleading or deceptive. For instance, a convincing enough visceralization that had subtly re-scaled data to exaggerate a certain effect may be taken at face value as true. Of course, this may be done intentionally for good purposes, such as how slow motion video is often used to emphasize high speeds, yet this comes at the expense of a less visceral understanding of the original speed that is being displayed. There has been extensive discussion of data visualizations potentially being deceptive, and special care needs to be likewise taken since data visceralization is intended to give an intuitive understanding of the data.% We have only begun to explore the effects of transforming data, and as noted in the previous section, have concluded that any scaling can potentially lead to deception.


\subsection{Concrete Scales within VR}
Since concrete scales relies on comparisons and re-scaling a semantically-understood anchor (or reference) objects, creating a concrete scale comparison in VR that re-scales the objects prevents the visceral understanding of the original measurements. As such, data visceralization can be seen as operating within a range of phenomena that can be conveyed directly to the viewer without re-scaling, i.e. the `perceptual sweet spot'. There may still be advantages of viewing concrete scales in a virtual environment, such as comparing sizes and shapes of buildings from multiple views to help understand their differences, but this is a separate phenomena from data visceralization.

%(these are just not data visceral experiences unless the objects remain at their original scales). As such, data visceralization operates within a narrow range of phenomena that can be conveyed directly to the viewer without scaling. There may be many advantages of viewing concrete scales in a virtual experience, for instance comparing the sizes and shapes of buildings from multiple views may help understand the differences, but this is a separate phenomena from data visceralization.

\subsection{Application Domains}
Since effective data visceralization restricts transformation of data, there are certain domains and experiences that are particularly well suited to data visceralization. We have already identified and demonstrated two prototypes using sports visualization, and this space could be explored more extensively. Scale comparisons of other human endeavors like architecture, engineering, and design are all enhanced by having deeper understanding of data. In particular, understanding the relative sizes of objects while browsing online services has been often suggested as a compelling use of immersive technology. Finally, there has been compelling video examples of the impact of weather events, like flooding, where a one-to-one demonstration of the height of the water, or the speed of windows being blown open, could help viewers more deeply understand what happens during the event. 

%Since we're limited in transforming data, there are certain domains and experiences that are particularly well suited to data-viscerlaization. We identified and showed several Sports Visualization examples, and this space could be extensively explored.
%Scale comparisons for other human endeavors such as architecture, engineering, and design are all enhanced by a deeper understanding of the data. In particular, understanding the relative sizes of objects that might be purchased from online services has been often suggested as a compelling use of VR technology. Finally, we have also seen video examples of the impact of weather events, like flooding, where a one-to-one demonstration of height of the water, or the speed of the windows, could help viewers more deeply understand the event. 


\subsection{Limitations of Visceralization}
\subsubsection{Technological}
Existing extended reality (XR) devices, which encapsulate augmented, virtual, and mixed reality (AR/VR/MR), have intrinsic technical limitations in terms of screen pixel dimensions, available field of view, and input capabilities. While these devices are now available for everyone beyond research purposes, there are still many technological factors to consider. Firstly, screen resolution, while not the strongest limiting factor per se (since available devices already display at sufficient resolutions to trigger the intended visceral effect) is an important factor. Better screen resolution will undoubtedly improve the quality and the quantity of displayed information. Secondly, the field of view is a crucial parameter which can hinder visceral perception within MR devices. In particular, users can be disturbed when a holographic object partially disappears upon reaching the boundary of the screen. This would disconnect the user with the mapping of the virtual object and their physical environment. Thirdly, interaction with the virtual or holographic environment can play a crucial role in the perception of visceralization. As stated, the one-to-one mapping with the user's motion and their environment must be maintained. This relies on accurate depth, motion perception and occlusion effects. When considering current technical limitations, user position tracking often becomes incoherent when the displayed information becomes too graphically demanding, which can cause latency in frame rate and thus breaks the one to one mapping. Future developments in this direction will provide the ability to run data visceralizations at a higher fidelity while maintaining high display frame rate.

\subsubsection{Perception in VR}
Much of the effectiveness of visceralization is based upon our capability to accurately perceive the virtual or mixed reality. While these technologies are capable of providing a vivid illusion of presence to users, there exist some limitations in how accurately people can perceive virtual stimuli as compared to in the real world. One such limitation relevant to our design probes is that egocentric distance estimations are compressed in VR \cite{Loomis:2003:VPE, Renner:2013:PED}, resulting in distance based visceralizations to be perceptually misleading. To combat this, the use of a virtual self-avatar has been shown to improve near distance estimation \cite{Ebrahimi:2018:IEA, Mohler:2010:TEV}. It has also been shown that the size of one's virtual body influences perceived world size \cite{Hoort:2011:BBT}, and the size of one's virtual hand influences perceived size of nearby objects \cite{Linkenauger:2013:WWT} which can in turn help improve size estimation \cite{Jung:2018:OMH}. As visceralizations are reliant on the accurate perception of virtual objects, these techniques and others similar in the VR literature can be leveraged.

\subsection{Future Work}
\subsubsection{Evaluation} 
We extensively discussed among the authors in critque sessions methods by which we could evaluate the effectiveness of data visceralization. This is particularly important when trying to compare what improves or interferes with data visceralization experiences (such as photo-realism or annotation). Some methods might correspond with experiments for testing the sense of presence in virtual environments such as those suggested in \cite{witmer1998measuring} \cite{Barfield:1995:PPW}. Beyond simply evaluating presence however, we  need to evaluate how well the data visceralization experienced helped in comprehending the underlying data. We speculated, through thought experiments, about learning transfer towards understanding measures in the real world, that is for example, would watching sprinters in a data visceralization then allow for their speeds to be accurately compared to those of real runners? While this might be a way of exploring the effectiveness of the experience, we have also noted that data visceralization is not about understanding exact measures and values, but instead to get an intuitive grasp of the phenomena, so simple time and accuracy studies would not be appropriate. Moreover, we have also discussed the effect of data transformations resulting in potentially deceptive experiences---how we measure such effects and their implications is unclear.

%Learning transfer, that is, does experiencing the phenomena in a VR setting allow one to improve performance in real life might be a way to explore the effectiveness of the experience. We speculated on thought experiments where we showed different sprinters in a data visceralization experience and then had someone judge the relative speed of a real runner. Unfortunately, as noted, data visceralization is not about comprehending exact estimates but more an overall, intuitive grasp of the phenomena, so precise time and accuracy experiments would not be appropriate. We have also extensively discussed the effect of transforming data leading to either non-visceral understanding of the data and potentially deceptive experiences. How might we measure such effects as well? 
 

\subsubsection{Interaction}
As we base our design probes on snippets of existing stories, their prototypes had rather limited interaction. In many cases, this was simply the ability to move around either freely or to preset way-points, toggle on or off certain visual variables (e.g. realistic vs primitive/abstract, annotations), or to play and pause time-dependent phenomena. As perception and interaction are intimately related, there are opportunities to explore how viscerality can be improved through increased interactions with the data, such as being able to influence a sprinter's performance based on additional variables like wind speed.

%Our current design probes had very limited interaction. We could move our viewpoint - both naturally using the headmount display and more artificially through jumping to preset viewpoints or placing the viewpoint on a moving object. We could also choose from  several preset modes that altered positions of objects in the environment or changed levels of realism. Since perception and interaction are intimately related, there are opportunities to explore how interaction might be used to improve a data visceralization experience.

\subsubsection{Mixed Reality}
As opposed to VR, MR (where real and virtual environments are blended together) offers its own opportunities and challenges. The most striking change is that the real-world acts as a baseline anchor for all measurements and scales. We foresee this as potentially vastly improving the familiarity and relatability of the data, as the experience is intrinsically linked to the user's environment and may be remembered as such. On the other hand, the real-world environment can limit the scales at which these experiences take place. For example, visualizing a life-sized skyscraper while inside of a building is impractical without some form of clipping or x-ray like vision, which may feel jarring to the user. Furthermore, current MR technology tends to have very narrow viewing regions which would further limit the scope of the experience.

\subsubsection{Extensions to Other Senses}
Researchers have explored how non-visual senses can be stimulated to convey data, such as olfaction (e.g., \cite{Patnaik:2019:IOH, Washburn:2004:ODI}) and gustation (e.g., \cite{Khot:2015:TDP}). Similar to data visualization however, these works still focus on transforming abstract data and mapping them along some sensorial channel \cite{McCormack:2018:MIA}, such as mapping arbitrary smells to colors in a network graph \cite{Patnaik:2019:IOH}. More closely related to the notion of visceralization is that done on haptic simulation \cite{Batter:1972:GCD, Brooks:1990:PGD:97880.97899}. Such systems allowed users to feel physical phenomena like magnetic fields or gravitational forces by using a force-feedback `haptic display'. Auditory displays (headsets) and sonification of phenomena has also been used to help transform data into sounds either for disabled participants or to help in understanding the abstract phenomena.

Many of these examples, particularly olfaction, gustation, and haptics/touch, are prototypes which are not yet available to the general public. Nevertheless, it is plausible that in the future, opportunities for multi-sensory data visceralization experiences will become ubiquitous. These could potentially provide much greater levels of presence and viscerality---through matching footfalls of sprinters, or leveraging smell which is known for its close association with memories.

%Some previous work been done on haptic experiences \cite{Brooks:1990:PGD:97880.97899}. Opportunities in other domains (sound, smell) and in sensory fusion - matching the footfalls of sprinters with the visual experience could help even more in viscerally understanding the data.

% On a related note, researchers have explored how non-visual senses can be stimulated to convey data, such as olfaction (e.g., \cite{Patnaik:2019:IOH, Washburn:2004:ODI}) and gustation (e.g., \cite{Khot:2015:TDP}). Similar to physicalization however, these works still focus on transforming abstract data and mapping them along some sensorial channel \cite{McCormack:2018:MIA}, such as mapping arbitrary smells to colors in a network graph \cite{Patnaik:2019:IOH}. More closely related to our work is that done on haptic simulation \cite{Batter:1972:GCD}. Such systems allowed users to feel physical phenomena like magnetic fields or gravitational forces by using a force-feedback `haptic display'. Auditory displays (headsets) and sonification of phenomena has also been used to help transform data into sounds either for disabled participants or to help in understanding the abstract phenomena. This work, however, focuses primarily on the visual senses, since except for audio, there are few commercial systems for these non-visual senses.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/Pipeline-Extended.png}
    \caption{This pipeline illustrates our data visceralization concept. The relevant physical phenomena is measured and stored accordingly as data. This data can either go through the the standard InfoVis pipleline \cite{Card:1999:RIV, Chi:1998:OIF}, or the Data Visceralization Pipeline, which optionally applies simulation, high/low fidelity rendering, and annotations to produce a final visceralization. These are aimed at mimicking the original physical phenomena as closely as possible, while complementing existing conventional data visualization.} 
    \label{fig:pipeline}
\end{figure}

\subsubsection{Developing a General Data Visceralization Pipeline}
Currently, all of our data visceralization design probes were created as special purpose, bespoke experiences. Development of these requires skills in design, 3D modeling, and programming in specialized environments such as Unity3D. Numerous development toolkits are emerging to make the construction of VR experiences easier without extensive programming experience. However given that data visceralization contains a data driven component, programming will likely still be involved in the future.  Based on our experiments, we found that we fell into the same patterns for each of the design probes we implemented which we portray in figure~\ref{fig:pipeline}. Akin to the InfoVis pipeline (and thus sitting in parallel to it), we take data directly into the Data Visceralization pipeline without transforming or aggregating it. That data is directly mapped onto attributes of an object within the virtual environment. In some circumstances (though not all) this may require some simulation of objects in the environment. For instance, in [EX1], our raw data consisted of time of completion for the 100m sprint. We used the speed to map the position of an object moving from the start to the end of the sprint. We simulated the motions of a runner to correspond with the motion of the object. Note well that these motions are simulated. If someone was trying to discover how subtle difference in movement made Usain Bolt a better runner, this would not be an appropriate experience, but it does help to understand the overall speed by which Bolt runs. After the objects are simulated, and an environment is created to contain them, we render them at different levels of realism. Finally, we optionally annotate the experience to add in some quantitative context for the experience. The output is then experienced on an appropriate VR (or MR) display. While nothing is currently automated in this pipeline, this structure helps organize where different contributions can occur.


==> sections/DeadText.tex <==
% from intro
%Similarly, other work has proposed personalizing data journalism by expressing distances or other quantities in terms of locally familiar references \cite{Hullman:2018:ICM}. %Alternatively, we introduce a method for directly experiencing the ground truth underlying a data visualization using augmented and virtual reality (AR/VR) which we call \textit{data visceralization}.
To complement and advance this line of research, we introduce \textit{data visceralization} as a method to allow people to directly experience the ground truth underlying a data visualization using augmented and virtual reality (AR/VR).

%Loosely, we define \textit{data visceralization} as the following:
%\begin{quote}
%    A data visceralisation is a data-driven experience which evokes visceral feelings within a user to facilitate intuitive understanding of physical measurements and quantities.
%\end{quote}

We introduce and define the term \textit{data visceralization} as a data-driven experience which evokes visceral feelings within a user to facilitate intuitive understanding of physical measurements and quantities. By visceral, we mean a 'subjective sensation of being there in a scene depicted by a medium, usually virtual in nature.' [ref Barfield, Woodrow; Zeltzer, David; Sheridan, Thomas; Slater, Mel (1995). "Presence and Performance Within Virtual Environments". In Barfield, Woodrow; Furness, III, Thomas A. (eds.). Virtual Environments and Advanced Interface Design. Oxford University Press. p. 473. ISBN 978-0195075557.]
% Interest in VR has seen a resurgence in recent years as the technology becomes cheaper, more advanced, and readily accessible to the general public. This commodification has spurred the research and development of VR for data visualization and analytics commmonly referred to as immersive analytics, though there still exists only scant evidence as to the effectiveness of 3D visualization to help communicate or understand abstract data. On the other hand, there is ample evidence to suggest that VR is effective for simulating realistic environments for a wide variety of uses such as immersive movies, psychological therapy, and military simulation \todo{refs}.
% As opposed to simply adding an extra dimension in common visualization types, AR/VR can be used to simulate the reality in which the data was originally measured from. Thus, users can gain a visceral understanding of the data by directly experiencing it. This addresses a specific shortcoming in common data visualization by leveraging one of the principal design goals of VR, the ability to simulate an alternate (virtual) reality as if it were a real experience. 
For example, while one has seen many illustrations of the relative heights of different buildings, it is hard to imagine the actual size of them unless one has seen them in person. Or alternatively, consider a news article about the relative speeds of olympic sprinters, we can see the times that it might take to perform a 100m race, but it's hard to tell what that means in terms of someone running by us.
By using VR, we can place a skyscraper, sprinter, or even a dinosaur directly next to us, allowing us to walk around the object and experience its size and other attributes directly relative to us. 
% on the ever increasing amount of garbage which ends up in landfills around the world. We can see illustrations of the amount of garbage (more than 2 billion tons each year), but how might we be able to experience these values first hand? Even drawings with a reference figure of a person requires a cognitive comparison of relative sizes, which must be learned. 
%We can be placed next to the mountain of garbage (and while olfactory simulation [ref] is still in its infancy [ref]), we can still get a deep understanding of the scope of the amount of garbage.

%\highlight{More formally, in this paper, we introduce the concept which we call \textit{data visceralization}---a data-driven experience which provides users a visceral understanding of physical measurements and quantities in order to complement a data visualization.}
In order to understand the circumstances when we can create effective data visceralization experiences, we built <n> prototypes for <x> different situations. We describe why we chose the particular prototypes, identify the range of phenomena that is appropriate for data visceralization, summarize under what situations they were effective (and when they were not effective) and discuss limitations and future work for this technology. 


% more dead textfrom intro

%OLD
\iffalse
\todo{flip around from vr focus to davaviz focus (steven's email)}
With the resurgence of virtual reality (VR), researchers and practitioners have been exploring how to best make use of the technology. One notable characteristic of VR is its ability to simulate convincingly realistic environments, actors, and objects at real-world scales with little to no added cost. This has seen many applications in fields such as military, medical training, and immersive storytelling.

VR has also been used for the purposes of data visualisation, exploration, and understanding, known as immersive analytics. Much existing work has focused on conventional visualisation idioms such as scatterplots and parallel coordinates plots, visualising these in various ways.

Data visualization as a whole is fundamentally about abstraction. It involves some process of measurement to generate data, which is then mapped to a chosen graphical representation. At each stage, abstraction is used to facilitate the communication of data.

As a result of abstraction, certain qualities of the original data are lost. This notion is especially true for measurements of physical properties (e.g., meters, gallons), where it can be difficult to comprehend the physical shape and/or sensation of the measurement.

Concrete scales---the process of visually re-expressing complex measures with familiar objects---is a common technique to aid in comprehension of physical measurements. However, this relies on readers' cognitive ability to build a mental model to properly conceptualise scale, requiring both time and effort. Applications of concrete scales have also been largely confined to 2D surfaces, found in media such as news articles, data videos, and infographics.

With VR, its aforementioned ability to simulate absolute scales allows us to bypass the need to re-express physical measurements as metaphorical units altogether. By simply recreating the original physical phenomena in VR, users can directly experience it as if they were actually there, leveraging their perceptive abilities.

While simulating objects may not improve the quantitative understanding of data---hence the need for measurements in the first place---the almost visceral experience of the data may aid in the \textit{qualitative} understanding of it. For instance, we know that Mount Everest is ~29,000 feet in elevation, and while many of us have seen pictures of the mountain, it is vastly different experience actually seeing it in person.

In this paper, we describe this process of understanding physical measurements through VR recreations as \textbf{data visceralisations}. While the term has been used to describe the invoking of emotions to enhance data communication, we take a broader approach by classing visceralisations as experiences which improve data understanding using \todo{give proper definition}.


\fi


%%%%%%%%%%%%%%%%%

\iffalse

% contributions
\todo{Reword at the end}
\begin{itemize}
    \item ground the work in the context of human perception of physical properties
    \item describe a series of examples demonstrating data visceralizations
    \item characterization of data visceralizations
    \item discussion of advantages, considerations and limitations
\end{itemize}

It is important to note that as data visceralizations are made possible through immersive technologies such as VR, the examples presented are not as effective on a flat 2D screen.


%%%% notes
-have shorter paper?
-do we focus on data stories? generate a corpus and see what \% of it is applicable
-include application domains as well
-interested in the absolute scales as that's what we're trying to visceralize, if it is outside of the sweetspot it might not be as visceral
-what is the definition of visceralisation? ecological psychology (gibson)
-keep pipeline to talk about examples, additional stages/processes when converting back from data to visceralisation
-design probes (the examples)
-lessons learned? critical reflection, look back on what we done in the examples
-examples are semi-experiments
-implications for design

-define domain
-show visualisation
-don't describe every single step
-of those what are the things worth sharing
-what was interesting things that we found!
-examples should be examples, the critical reflection is looking back and pointing out things we did that are worth mentioning

-probe 1
-reflection 1
-probe 2
-reflection 2
-etc...


%%%%%% other notes
- concrete scales and one-to-one preserved mappings: one-to-one is what we retain as the most visceral experiences. concrete scales can still be used to retain the semantics of the data but can lose the visceral experience
- applicability of scientific visualisation to visceralization


%%%%% more other notes
- add original version of the data stories and visualisations, get permission later on
- future work: understand the mapping of these experiences, for automated pipeline

- related work in vr and visceralization


main points left to include:
- why these examples are chosen
- scaling and viscerality, scaling causes issues with viscerality, collapses down into an experience you can have on another device such as a screen


why these examples were chosen:
- the runners down the track (data story) was the most directly related to VR as it was closest to reality
- we talk about it in the context of data stories as we dont have to add all that extra context

going from good examples into negative examples
1. sprinters
2. long jump
3. skyscrapers
4. solar system
5. protests
6. us debt

-> do top down approach?
- focus on the senses and talk about senses from there
- we thought things would be good examples but it turned out they werent
- out of the list of compatible things, we chose 

we're looking for a class of examples that has not been abstracted into a scatterplot

maybe start with building example?

- how do we isolate viscerality?



video:
todays data videos are like this, however we can experience them like this!
show contrast of how data is usually represented, future
talk about the progression from source, abstraction, closer to experience, to visceralization
define the concept of visceralization at the end


\fi









\subsection{Information Visualization and Visceralization}
In conventional data visualization, raw data undergoes a series of transformations and mappings until a visualization is rendered and created \cite{Card:1999:RIV, Chi:1998:OIF}. To better understand how data visceralizations relate to regular data visualization, figure~\ref{fig:pipeline} shows a modified version of the infovis pipeline \cite{Card:1999:RIV, Chi:1998:OIF}. Firstly, it includes an additional stage before the raw data, which we refer to as physical phenomena. This is the distal stimuli \cite{Jerald:2015:VBH}---some actual object and/or event in the world that is of interest. It is then measured to produce the initial raw data, stored as a magnitude unit pair (e.g., 23 kilograms, 6 feet). Secondly, the processed data during the pipeline can be instead used to recreate the original physical phenomena. This mimicry aims to create an artificial version of the distal stimuli such that the proximal stimuli \cite{Jerald:2015:VBH} is convincing enough to evoke the visceral sensation of properly experiencing it. Important to note is the reliance on \textit{physical} phenomena. More conceptual and abstract types of data, such as movie ratings and life expectancy, do not have direct physical equivalents and therefore are not applicable.




\subsection{Viscerality in VR}
- real life simulations for phobias, training, etc.

\subsection{Visual perception in virtual reality}
- depth perception accuracy
- movement perception accuracy
- scale perception accuracy

\subsection{Ranges of Human Perception}
\todo{fill in}
While VR is capable of simulating objects of any size, speed, or shape, it is unreasonable to do so at extreme magnitudes due to the limits of human perception. This is known as \textbf{psychophysics}. Take for example:
- bullets move far too fast to even be visible to the naked eye;
- an object moving at 1000km/h would look no different than 1050km/h;
- a 20,000ft tall mountain would invoke the same response as a 25,000ft tall mountain.

This is important to consider depending on the intent of the visceralisation. For example:
- if the purpose is to show how heavy something is to the point where you can't pick it up, then it is perfectly fine if the user can't pick it up;
- if the purpose is to just show the raw value of something such as height of a building, then this may also be acceptable;
- if the purpose is to compare between different values, then this needs to be considered

These ranges are not set in stone and may be different from person to person, however there might be a sweet spot.






\subsection{Multisensory Data Visualisation and Data Physicalization} \label{ssc:multisensory-datavis}
As data visceralizations aim to give users a visceral understanding of physical properties, it is apparent that they can extend beyond sight, as is necessary to experience data such as temperature and weight. Along these lines, researchers have been exploring how data can be explored and presented `beyond the desktop'---both in terms of visual display devices \cite{Marriott:2018:IA}, and to utilize the rest of our senses including touch/haptics (e.g., \cite{Jansen:2015:OCD, Menelas:2014:VRT, Prouzeau:2019:SHI, Ogi:1996:MDS}), smell (e.g., \cite{Patnaik:2019:IOH, Washburn:2004:ODI}) and taste (e.g., \cite{Khot:2015:TDP}) . To formalize how senses relate to data, McCormack et. al provide a design framework for multi-sensory immersive analytics \cite{McCormack:2018:MIA}. They define a \textit{sensorial mapping} as ``a mapping from data elements and data attributes to sensory channels and their respective sensorial variables'', in a similar manner to traditional data visualization and its geometric elements \cite{Munzner:2014:VAD}. While this mapping can technically be chosen arbitrarily, they advise that certain mappings will be more effective than others due to characteristics of the human sensory system or device limitations. In the case of data visceralizations, it is clear that choosing a mapping that correctly portrays the source of the data would result in the most viscerally accurate sensations.

Data physicalization is a closely related field which explores how data can be encoded and presented using physical artifacts \cite{Jansen:2015:OCD}. Physicalizations are tangible, real-world objects which inherently utilize non-visual senses (most notably touch) to convey a much broader range of information such as texture. Given enough resources and advancements in technology, physicalization theoretically encompasses the visceralization space as any physical phenomena can be fabricated and simulated. However, existing research has focused on physicalizations as tangible representations of abstract data and concepts such as 3D bar charts \cite{Jansen:2013:EEP, Taher:2017:IUD}, as well as other non-academic examples found on the list of physical visualizations\footnote{http://dataphys.org/list/}. Moreover, much of the technology which enables physicalization can consequently be used for visceralization. \todo{i'm not sure how to close this out...}


\subsection{Understanding Physical Measurements}
Although not strictly tied to data visualization, concrete scales are commonly used to better help comprehend physical measurements. 

While not exactly concrete scales, size diagrams / police line-ups / identity parades / whatever they're called can help to understand physical measurements by contextualizing it in relation to other related units, such as similar species of animals or the average human person.

Transforming data into more familiar units can also be done. For instance, rates of distance change is oftentimes transformed back into time for both speed (e.g., race times) and acceleration (e.g., 0 to 100 kmph). These involve some level of recontextualization, framing a transformed measurement in the context of another. For example, rather than saying the car accelerated at 4 meters per second per second, we frame it in the context of to travel from a speed of 0 kmph to 100 kmph, it takes 4 seconds.


\subsection{Gibson User Environment Understanding}
Gibson defines the human perception system \cite{Gibson1979-GIBTEA} no only based on a projected image on the retina but rather with a global system with eye attached to the head with the neck for rotation and the legs for locomotion. In his perception model, user surrounding understanding is tightly linked to the body movements. In this sense, head mounted display devices, and their ability to display a 3D view which is directly connected to user movement, is compliant to the Gibson model with invariants and affordances.

The human perception changes when the user moves but some information remains the same. These so called invariant correspond to theses structures which maintain specific visual properties when the user moves in his environment. For example, the user do not need to move to perceive a table (compose of many invariant sharp angles), but the user have to move to learn what a table is. This notion is close to the concrete scale understanding and can model the user learning process. Affordances is a more elaborate perception phenomenon and it can be considered has invariant of invariant. Something that does not change as all (i.e. a door  or a tree).


\section{Data Visceralizations in Virtual Reality} \label{sec:perception}
As previously stated, it is theoretically possible to fabricate and simulate all visceralizations as data phsyicalizations. This is oftentimes not the case however, as issues such as fabrication time and space restrictions will always play a factor. We foresee VR as a suitable and effective means of achieving these visceral experiences. This is due to, and not limited to: there being near infinite possibilities for visual display at little to no additional cost; does not require any additional setup outside of launching the experience itself; and it allows users who already own VR devices to enjoy them in their own homes.

We expect that achieving viscerality would be dependent on technology and processes used to simulate the experience. With VR, it is capable of effectively supporting both vision and sound. Many consumer VR devices offer handheld controllers which provide haptic vibration and feedback, but are limited in comparison to vision and sound. There do exist prototypes which aim to provide much better haptics, such as TORC \cite{Lee:2019:TVR} and the HaptX Gloves\footnote{https://haptx.com/}, and even other prototypes for smell such as viScent \cite{Patnaik:2019:IOH} and those listed in \cite{Washburn:2004:ODI}. However, these are all not readily available to consumers nor the general public, therefore we exclude them from our work.

Data visceralizations rely on our perceptive abilities to properly take in and experience stumili. Given that VR relies heavily on vision to immerse the user in an alternate environment, we discuss human perception capabilities in relation to sight. \todo{include something here about how visceral reactions are beyond our cognitive control, and therefore if we dont accurately perceive the sensations then these reactions will not be triggered}





As stated in section on\todo{perception section}, there are certain ranges which humans can accurately and readily perceive physical phenomena. Those within this range can be said to be in a `sweet-spot', and can be simulated and perceived as-is without additional changes. These are oftentimes human-scale, and due to their familiarity can be said to evoke the most visceral experiences. Physical phenomena outside of this range however may not be as directly perceivable, therefore impacting both viscerality and data understanding. Data visceralization works best on ranges and for comparisons in this perceptual sweet-spot which means that it's not applicable to all visualizations. It's also not necessarily appropriate for illustrating abstract concepts such as money, feelings, life expectancy, etc. While this can be limiting, there are certain domains, such as sports statistics, human-scale biology, architecture and small level city planning, localized weather phenomena (flooding, wind) all operate in this sweet spot of human perception and can be enhanced with data visceralization.


We discuss techniques for resolving this based off our design probes and other related fields.



\subsubsection{Re-expression through concrete scales}
There may be occasions where there exists little to no possibilities for accurate rescaling. For example, microbial or even atomic sized phenomena cannot be experienced without some form of magnification. Concrete scales \cite{Chevalier:2013:UCS} is one common approach used to help comprehend these extreme magnitudes, using either textual or pictorial analogies. \todo{add definition if not in related work} While mostly found in 2D images and text, the concept can easily be applied in data visceralization. In VR with vision, life-sized 3D models can be used in place of 2D images. While the original phenomena may not be experienced viscerally nor accurately, users can get an accurate sense of the re-expression unit as compared to just a picture (e.g., what type of orange and how big is it?).

\subsubsection{Intentionally keeping things out out percepibility} 
In spite of the aforementioned techniques, there may be some instances where it is intended to keep things imperceivable. In this case, it is reasonable to not apply any scaling or re-expression techniques and to leave it as is. For example, a story about the Great Pacific Garbage Patch may choose to show its extent simply by showing the garbage all the way to the edge of the horizon as it may be in reality. While the user may not be able to perceive and understand exactly how much garbage there is floating in the ocean just by looking at it, there can still be the visceral effect of acknowledging the amount of garbage there is, thus prompting them to take action.

\subsection{Changing perspectives for unique insights}
A key motivation for the use of data visceralization is to understand physical measurements and phenomena in a unique manner not otherwise possible on conventional 2D screens. While this remains true during our design probes, we realized that VR also encourages experiencing unconventional perspectives attain more nuanced insights. For example in EX1, while many stories about sports would compare and contrast the different athletes with one another based off their results, we can instead experience what it may be like to be one of the athletes competing against the others. While it is certainly possible to create conventional data stories in such a manner which supports this, we feel that VR makes this process more appealing and organic---if you are already at the bottom of the Empire State Building, what would it be like to be at the top? This may drive both memorability and engagement during the story.

\subsection{Annotations and immersion}
Data visceralization aims to improve the qualitative understanding of data by essentially simulating its source. By doing so, some of the basic benefits of abstract quantitative understanding can be lost as it becomes difficult to accurately estimate physical properties \todo{find sources if this is true}, hence the utility of the data visualization in the first place. Visceral experiences can be augmented with labels, highlights, and annotation.  This can be done either by simply informing the user before they experience the (phenomena?) data, or by overlaying the annotations in-situ on top of the relevant stimuli \cite{Willett:2017:EDR, Thomas:2018:SA}. 
%The latter is a compelling application which further leverages the virtuality of VR, minimizing the need for users to redirect their attention from stimuli to data. 
However, this can potentially be distracting and harm the immersiveness of the experience. %more here


\subsection{Usefulness of realism}
In all of our examples, we allow the scene to change from realistic looking models to simple shape primitives.  This raises a question on the purpose of realism in data visceralization: is it necessary for a representation to be realistic if the underlying data can still be understood? For example, does data about volume need to be accompanied by an exact 3D replica of the object at hand? Of course, there are certain instances where realism is absolutely imperative, such as the New York Times' piece on Olympic athletes in AR \cite{NewYorkTimes:2018:OlympicAthletes}.

\subsection{Contextual Backgrounds}
While initially not doing so, we decided to add appropriate 3D models and detail to the background. This was done to improve perception of the intended stimuli. However, this may have other additional effects, most notably improving context and memorability of the experience. %more here: preattentive processing, ecological psychology?, chartjunk


\subsection{Learning transfer towards actual reality}

\subsection{Challenges in implementation}
While data visualization practitioners are very experienced in conventional tools such as D3.js and R, data visceralization demands a different skill set, including but not limited to 3D graphics, modelling, and human perception.

In addition, the devices required to accomplish such visceralizations such as VR are no where near the level of ubiquity that monitors, phones, and tablets are, This severely limits the audience capable of consuming these experiences, which can be a deciding factor when deciding to create them.

How visceralizations are accessed and their interplay with visualization would have a profound impact on their effectiveness while out-in-the-wild. Take a data story with VR for example. Designers may decide to use a visceralization purely complementarily, giving readers the option to put on their VR headset at specified moments to `experience the data for yourself.' Alternatively, they may instead decide to use VR to tell their entire story, interweaving these visceral experiences with other immersive storytelling elements \cite{Bastiras:2017:CVR,Ren:2018:XIC}.


==> sections/alt-text.tex <==
Figure 1: Four separate images organized in a 2 by 2 grid. First image is a screenshot of a table of results from the Olympic Men's 100m, with names of each sprinter and their sprint times next to it. Second image is a screen capture of a data visceralization running in virtual reality based on the previous image, showing more than 10 3D models of athletes running down a 100m track at a real-life scale. Third image is of a comparison diagram with silhouettes of different skyscrapers lined up next to each other with a y-axis for height. Fourth image is a screen capture of a data visceralization running in virtual reality based on the previous image, showing real-life scale models of the Eiffel Tower, Space Needle, and the Eiffel Tower.
Figure 2: Six separate images organized in a 2 by 3 grid describing EX1. First image is a screen capture of the original data story's video which our design probe is based off, showing more than 10 3D models of athletes running down a 100m track. Second image is a screen shot of more than 80 3D models of runners in VR running down the track. Third image is an equivalent screen shot but with white cubes instead of models of runners. Fourth image is of a first person perspective of the slowest runner along the track. Fifth image shows the runners with annotations above their heads stating their names, their sprint time and their speed. Sixth image shows all runners superimposed on top of one another in a single lane.
Figure 3: Four separate images organized in a 2 by 2 grid describing EX2. First image is a screen capture of the original data story's video which our design probe is based off, showing a top down view of arrows representing distance jumped by Olympic long jump medalists overlaid by a basketball 3-point line. Second image is a still frame of 80+ 3D models of long jumpers in VR. Third image is a close up version of this still frame. Fourth image shows the distances each long jumper jumped superimposed on top of one another, represented instead by small flags with annotations above the farthest and closest flags.
Figure 4: Six separate images organized in a 2 by 3 grid describing EX3. First image is of a viewpoint from below the Eiffel Tower at ground level looking up towards its top in VR. Second image is of a viewpoint from the top of the Statue of Liberty looking up towards the Space Needle nearby. Third image is of the foundation of the Statue of Liberty with real-sized human models walking around its base. Fourth image shows shadows being cast from one skyscraper to the next from a light source directed parallel to the ground. Fifth image shows a miniature version of the data visceralization, with the 5 skyscrapers lined up side by side. Sixth image shows a zoomed out version of the data visceralization, with the 5 skyscrapers lined up side by side but off in the far distance.
Figure 5: Two separate images side by side describing EX4. First image is a computer graphic of all the planets in the solar system lined up side by side next to each other, with the Earth and Moon on either end, illustrating that all other planets can fit between the Earth and the Moon. Second image is a VR equivalent using scaled down 3D models.
Figure 6: Four separate images organized in a 2 by 2 grid describing EX5. First image is a screen capture of the original data story which shows birds-eye view pictures of the Hong Kong protests. Second image is a VR equivalent showing the viewpoint of being in the middle of a crowd of 3D life-sized human models along a road. Third image is from a viewpoint above the crowd in a helicopter with its shadow clearly visible. Fourth image is of a similar viewpoint but with human-sized cubes instead of 3D models.
Figure 7: Four separate images with one larger image and three smaller ones to the side describing EX6. First image is a screen capture of the original data story illustrating the amount of debt the US has represented as $100 dollar bills in large stacks around the Statue of Liberty. Second image is a VR equivalent showing these stacks surrounding the Statue of Liberty. Third image is from a viewpoint standing on top of one of these stacks looking down from above. Fourth image is from a viewpoint at ground level looking up towards the tops of the $100 bill stacks and the Statue of Liberty.
Figure 8: Diagram illustrating the difference in perception when looking at a scaled down object from up close versus from afar. It shows an eye representing the viewer with a cone protuding away from it representing the viewer's field of view. One icon of a building labeled as scaled down is positioned close to the eye, with another similar icon labeled as 1:1 scale is positioned further away from it. Semi-transparent versions of the eye and cone offset vertically by a small amount demonstrate the effect that movement has on the perception of these buildings. Smaller boxes appear below the scaled down building showing a large difference in position between an opaque building and the offset transparent version, amd the 1:1 scale building showing a smaller difference.
Figure 9: A flow chart demonstrating the data visceralization pipeline. It begins at physical phenomena which is measured and turns into data. This data then feeds into either the InfoViz Pipeline or the Data Visceralization Pipeline. The InfoViz pipeline is intentionally hidden away and leads straight into Data Visualization. The Visceralization pipeline includes three optional stages: simulation, rendering, and annotation. This pipeline then leads into the final Data Visceralization stage. Dotted lines also connect Data Visceralization and Data Visualization stating "complements", and another line from Data Visceralization and Physical Phenomena stating "Mimics.

==> sections/cover-letter.tex <==
Dear Reviewers,

Our paper was previously submitted for ACM CHI 2019 and IEEE VR 2019 (previously submitted manuscript and reviews attached). While reviewers praised the novelty and discussion of the concept of "data visceralization" presented in the paper, they saw the lack of external user feedback to be too hard to ignore, as the majority of discussion was given from the viewpoint of the authors. They suggested that including some form of external feedback and opinion—even if minimal, informal, or subjective—would result in a much stronger submission.

To resolve this, we ran sessions with external users where they experienced our data visceralization prototypes for themselves.  We gathered their responses and opinions. Note that as past reviewers suggested, we do not conduct these as formal user studies, but instead use them to further guide and refine the concept. As a result, we were able to expand on our existing discussion of data visceralization with similar/opposing feedback, identify a set of new themes and considerations for the concept which we did not have previously, as well as better define our directions for future work.

Kind regards,
The authors
